Probabilistic bounded reachability for hybrid systems with continuous nondeterministic and probabilistic parameters

We develop an algorithm for computing bounded reachability probability for hybrid systems, i.e., the probability that the system reaches an unsafe region within a finite number of discrete transitions. In particular, we focus on hybrid systems with continuous dynamics given by solutions of nonlinear ordinary differential equations (with possibly nondeterministic initial conditions and parameters), and probabilistic behaviour given by initial parameters distributed as continuous (with possibly infinite support) and discrete random variables. Our approach is to define an appropriate relaxation of the (undecidable) reachability problem, so that it can be solved by $\delta$-complete decision procedures. In particular, for systems with continuous random parameters only, we develop a validated integration procedure which computes an arbitrarily small interval that is guaranteed to contain the reachability probability. In the more general case of systems with both nondeterministic and probabilistic parameters, our procedure computes a guaranteed enclosure for the range of reachability probabilities. We have applied our approach to a number of nonlinear hybrid models and validated the results by comparison with Monte Carlo simulation.

==> bbal.tex <==
As an example of a hybrid system described above we consider the following scenario (Figure 1): 
the ball is launched from the initial point with initial speed $\upsilon_0$ and angle 
to the horizon $\alpha$. When the ball reaches the ground it reflects according to the laws 
of reflection.

\begin{figure}[ht!]
\centering
\includegraphics[width=90mm]{bouncing-ball.jpg}
\caption{Bouncing ball scenario}
\end{figure}

The ball trajectory is defined by the system of equations:
\begin{equation} \label{eq:Sx}
S_x(t) = S_{x_0} + \upsilon_0 t \cos{\alpha}
\end{equation}
\begin{equation} \label{eq:Sy}
S_y(t) = S_{y_0} + \upsilon_0 t \sin{\alpha} - \frac{g t^2}{2}
\end{equation}
where $S_x$ and $S_y$ are projections (on the axes $x$ and $y$, respectively) of the distance travelled by the ball starting at the point $(S_{x_0}; S_{y_0})$, $\upsilon_0$ is the initial speed, $\alpha$ is the angle to the horizon, $g$ is standard gravity and $t$ is time. In this example we assume that the initial point of the ball's centre is $(S_{x_0} = 0; S_{y_0} = 0)$

A hybrid system characterising the behaviour of the ball will consists of a single mode with the dynamics defined in (\ref{eq:Sx}) and (\ref{eq:Sy}) and the only jump to the same mode, during which the time $t$ is reset to $0$, the value of $S_x(t)$ before the jump is assigned to the initial value of $S_x(t)$ in the mode after the jump, and the speed of the ball is reduced by the coefficient $0.9$.

In order to comply with the description of the hybrid system with random continuous initial parameters, let $\alpha$ be uniformly distributed over the interval $[0, 0.5]$ with the probability density function $f_{A}(\alpha) = 2$. Let $\upsilon_0 = 20$ and $t \in [0, 3]$.

Let us consider a bounded probabilistic reachability problem: \textit{is the probability that 
the system reaches in 4 steps the box $D =  \{S_x \in [90, 91], S_y \in [1, 2]\}$ greater or equal 
to $0.062$}?

The Borel set of continuous parameters is formed as:
\begin{equation*}
\begin{split}
B =\{\alpha: \exists t_{0, q_0}, t_{1, q_0}, t_{2, q_0}, t_{3, q_0} \mathord{\in} [0, T]:\\
(S_{x0} = \upsilon_0 t_{0, q_0} \cos{\alpha}) \\
\wedge (S_{y0} = \upsilon_0 t_{0, q_0} \sin{\alpha} - \frac{gt_{0, q_0}^2}{2}) \wedge 
(S_{y0} = 0) \wedge (t_{0, q_0} > 0) \\
\wedge (S_{x1} = S_{x0} + 0.9 \upsilon_0 t_{1, q_0} \cos{\alpha}) \\
\wedge (S_{y1} = 0.9 \upsilon_0 t_{1, q_0} \sin{\alpha} - \frac{gt_{1, q_0}^2}{2}) \wedge 
(S_{y1} = 0) \wedge (t_{1, q_0} > 0) \\
\wedge (S_{x2} = S_{x1} + 0.9^2 \upsilon_0 t_{2, q_0} \cos{\alpha}) \\
\wedge (S_{y2} = 0.9^2 \upsilon_0 t_{2, q_0} \sin{\alpha} - \frac{gt_{2, q_0}^2}{2})
\wedge (S_{y2} = 0) \wedge (t_{2, q_0} > 0) \\
\wedge (S_{x3} = S_{x2} + 0.9^3 \upsilon_0 t_{3, q_0} \cos{\alpha}) \\
\wedge (S_{y3} = 0.9^3 \upsilon_0 t_{3, q_0} \sin{\alpha} - \frac{gt_{3, q_0}^2}{2}) \wedge \\
(S_{x3} \in [90, 91]) \wedge (S_{y3} \in [1, 2])\}
\end{split}
\end{equation*}

Functions $S_x(\alpha, t)$ and $S_y(\alpha, t)$ are invertible with respect to $\alpha$ on 
the domain $[0, 0.5]\times[0, 3]$. Then by applying Proposition \ref{prop:ivp} the formulated 
reachability problem can be encoded as a SMT formula and solved using dReal:
\begin{multline*} 
\exists \alpha \in B = [\alpha_{min}, \alpha_{max}]:\\
(F_A'(\alpha) = f_A(\alpha)) \wedge (F_A(\alpha_{min}) = 0) \wedge (F_A(\alpha) \ge 0.062) .
\end{multline*}
The actual dReal output on the formula above was as follows:
\begin{verbatim}
SAT with the following box:
 time_0:[0.03127620501613272,
                         0.03127624003371717]
 Fa_t:[0.0625524053632542,
                         0.06255247702735234]
 Fa_0:0
 a_0:[0.4292134593911809, 0.4292134922320248]
 t_10:[1.528734841443786, 1.528734859618606]
 t_20:[1.37586135729942, 1.375861377493665]
 t_30:[1.042516533544058, 1.042516555982107]
 t_0:[1.813824229846001, 1.813824261219404]
 t_1:[1.632441880862484, 1.63244191572182]
 t_2:[1.46919748799121, 1.469197526723806]
 t_3:[0.8312598060237518, 0.8312598490599685]
 t_00:[1.698594379660991, 1.698594396018329]
 a_t:[0.4604896994248981, 0.460489732265742]
\end{verbatim}

The probability of reaching the unsafe region by the system thus falls into the interval 
$[0.0625524053632542, 0.06255247702735234]$, that is, the interval associated to the final 
value of $F_A$ (corresponding to \verb#Fa_t# in the printout above). The obtained result was 
validated using a simple Monte Carlo method in MATLAB. The time variable was discretised over 
the interval $[0, 3]$ and the system was simulated using 10,000 uniformly random samples from 
the interval $[0, 0.5]$. The number of samples hitting the unsafe region was 620, thereby 
giving a {\em probabilistic} estimate of $\frac{620}{10,000}= 0.062$. In comparison, our method 
gives an interval of size $0.72\times 10^{-7}$ which is {\em guaranteed} to contain the actual 
probability.



==> integrate.tex <==
In order to compute probabilistic reachability in hybrid systems with unbounded random parameter it is sufficient to solve bounded $\Sigma_1$ sentences of the following type:
\begin{equation} \label{eq:integration-problem}
\exists x \in [a, b] : \int_{a}^{x} f(t)\, dt \ge C
\end{equation}
for some constant $C\in [0,1]$.

\begin{proposition} \label{prop:ivp}
Let $f\mathord{:}[a,b] \rightarrow \mathbb{R}$ be a Lipschitz-continuous function. Then there 
exists one and only one continuous and differentiable function $F$ on $[a, b]$ 
such that $F(a) = 0$ and $\forall x \in [a, b]: \int_a^x f(t)\, dt = F(x)$
\end{proposition}

\begin{proof}
Let us formulate an initial value problem:
\begin{equation} \label{eq:IVP}
(F'(x) = f(x)) \wedge (F(a) = 0)
\end{equation}
where $f(x)$ is Lipschitz-continuous in $F(x)$ and continuous on $[a,b]$. 
By the Picard-Lindel\"{o}f theorem and the assumption $F(a)=0$, the formulated IVP 
has a unique solution on $[a, b]$ derived as following:
\begin{equation*} 
\forall x \in [a,b]: \int_a^x f(t)\, dt = F(x) - F(a) = F(x)
\end{equation*}
\end{proof}

Proposition \ref{prop:ivp} allows assessing the value of the integral by the value of the 
function which is obtained from the initial value problem (\ref{eq:IVP}). Therefore, 
the integration problem (\ref{eq:integration-problem}) is equivalent to the sentence
\begin{equation*} %\label{eq:encoding}
\exists x \in [a, b] : (F'(x) = f(x)) \wedge (F(x) \ge C) \wedge (F(a) = 0)
\end{equation*}
which can be directly solved by dReal as a $\delta$-satisfiability problem.



==> multivar.tex <==
\section{Multiple random variables}
In this section we discuss the enhancements to the proposed algorithm for solving probabilistic bounded reachability in hybrid systems with multiple independent random continuous initial parameters. Essentially, the structure of the algorithm will remain the same but the error estimation and box division strategy will be changed.

\subsection{Error estimation}
In order to calculate the probability of reaching an unsafe region by a hybrid system with multiple independent continuous random initial parameters, it is sufficient to obtain a Cartesian product of partitions over each random variable and verify each {\em box} from the Cartesian product.
\begin{proposition}
Given a hybrid system with $l$ independent continuous random initial parameters and a desired size of the probability interval $\epsilon_{prod} \in \mathbb{Q}^{+}$ each random variable should be integrated with precision $\epsilon$ satisfying the formula below:
\begin{equation} \label{eq:multivarmaininequalityspecialcase}
\begin{split}
\epsilon_{prod} \le {{l}\choose{1}}\epsilon + {{l}\choose{2}}\epsilon^{2} + ... + {{l}\choose{i}}\epsilon^{i} + ... + {{l}\choose{l-1}}\epsilon^{l-1}  + {{l}\choose{l}}\epsilon^{l}
\end{split}
\end{equation}
where ${{l}\choose{i}}$ - binomial coefficient.
\end{proposition}
\begin{proof}
If a hybrid system has $l$ independent initial random parameters then the probabilistic reachability can be computed as:
\begin{equation} \label{eq:mulvar}
\int_{B} \prod_{i = 1}^{l} dP(r_{i})
\end{equation}
where $dP_{i}$ is a probability measure of the $i$-th random parameter and $B$ is a Borel set such that $B = [a_{1}, b_{1}] \times ... \times [a_{l}, b_{l}]$ containing all the values of random parameters for which the hybrid system reaches the unsafe region.

We can employ the technique described above for computing the formula (\ref{eq:mulvar}). The formula will be presented in the form:
\begin{equation} \label{eq:mulvarind}
\int_{\Omega} I_{B}(r_{1}, ..., r_{l}) \prod_{i = 1}^{l} dP(r_{i})
\end{equation}
where $I_{B}(r_{1}, ..., r_{l})$ is the indicator function which is equal to 1 if the system reaches the unsafe region and 0 otherwise.

Using the definition of the indicator function the formula (\ref{eq:mulvarind}) is equivalent to
\begin{equation}
\int_{\Omega} \prod_{i = 1}^{l} dP(r_{i})
\end{equation}
for all $r_{i}$ for which the system reaches the unsafe region. The value above can be calculated as a product of the integrals.

\begin{equation}
\int_{\Omega} \prod_{i = 1}^{l} dP(r_{i}) = \prod_{i = 1}^{l} \int_{a_{i}}^{b_{i}} dP(r_{i}) = \prod_{i = 1}^{l} I_{i}
\end{equation}

Now it is desired for the product of the integral to be contained in the interval of defined length $\epsilon_{prod}$. Taking into account that we can obtain an interval of length $\epsilon_{i}$ containing its {\em exact} value of the $i$-th integral its sufficient to demonstrate how the values $\epsilon_{i}$ should be chosen so that the product of integrals is contained within the interval of length $\epsilon_{prod}$.

According to the rules of interval arithmetics product of the integrals is contained in the interval:
\begin{equation}
[\prod_{i = 1}^{l} I_{i}^{est}, \prod_{i = 1}^{l} I_{i}^{est} + \epsilon_{prod}] = [I_{1}^{est}, I_{1}^{est} + \epsilon_{1}] \cdot ... \cdot [I_{l}^{est}, I_{l}^{est} + \epsilon_{l}] = [\prod_{i = 1}^{l} I_{i}^{est}, \prod_{i = 1}^{l} (I_{i}^{est} + \epsilon_{i})]
\end{equation}

Therefore, given $\epsilon_{prod}$ the values of $\epsilon_{i}$ should be chosen in such a way that the following inequality holds:
\begin{equation} \label{eq:mulvarinequality}
\prod_{i = 1}^{l} I_{i}^{est} + \epsilon_{prod} \le \prod_{i = 1}^{l} (I_{i}^{est} + \epsilon_{i})
\end{equation}

\iffalse
Let $R$ denote a set $\{I_{1}^{est}, ..., I_{n}^{est}\}$ and $S = \{\epsilon_{1}, ..., \epsilon_{n}\}$. Then the right-hand side of the formula (\ref{eq:mulvarinequality}) can be modified:
\begin{equation}
\begin{split}
\sum ({{R}\choose{0}}{{S}\choose{l}}) + \sum ({{R}\choose{1}}{{S}\choose{l - 1}}) + ... + \sum ({{R}\choose{i}}{{S}\choose{l - i}}) + \\
... + \sum ({{R}\choose{l - 1}}{{S}\choose{1}}) + \sum ({{R}\choose{l}}{{S}\choose{0}})
\end{split}
\end{equation}
where $\sum ({{R}\choose{i}}{{S}\choose{l - i}})$ is a sum of products of all the combinations of length $i$ from the set $R$  multiplied by the combinations of length $l - i$ from set $S$ chosen in such a way that all the indexes in each of the obtained products do not repeat. 

Taking into account that $I_{i}^{est} \in [0, 1]$ the following holds:
\begin{equation} \label{eq:multivarmaininequality}
\begin{split}
\epsilon_{prod} \le \sum {{S}\choose{l}} + \sum {{S}\choose{l - 1}} + ... + \sum {{S}\choose{l - i}} + \\
... + \sum {{S}\choose{1}} + \sum {{S}\choose{0}}
\end{split}
\end{equation}
\fi

Therefore, choosing $\epsilon_{i}$ in such a way that (\ref{eq:mulvarinequality}) holds will guarantee that the {\em exact} value of the product of $l$ integrals is contained in the interval of size $\epsilon_{prod}$. In a special case when all $\epsilon_{i}$ are equal to $\epsilon$ the formula (\ref{eq:mulvarinequality}) can be simplified:
\begin{equation} \label{eq:multivarmaininequalityspecialcase}
\begin{split}
\epsilon_{prod} \le {{l}\choose{1}}\epsilon + {{l}\choose{2}}\epsilon^{2} + ... + {{l}\choose{i}}\epsilon^{i} + ... + {{l}\choose{l-1}}\epsilon^{l-1}  + {{l}\choose{l}}\epsilon^{l}
\end{split}
\end{equation}
where ${{l}\choose{i}}$ is a binomial coefficient
\end{proof}

\subsection{Division strategy}
Given a box $D = [a_{1}, b_{1}] \times \cdot \times [a_{n}, b_{n}]$ we can partition it into $2_{n}$ boxes of the equal sizes in such a way that each interval $[a_{i}, b_{i}]$ is altered. This procedure should be applied to every box for which decision procedure defined above returns \textbf{$\delta$-sat} for both formulas until the desired precision is reached.

\begin{remark}
Essentially, any division strategy can be applied as long as the size of each interval forming the box is reduced.
\end{remark}



==> onerand.tex <==
In the scope of this paper we consider hybrid systems with one random initial parameter, and 
we propose an algorithm solving the probabilistic $\delta$-reachability problem for such 
hybrid systems. In a hybrid system with random parameters, the random variable $r$ is defined 
over a bounded interval. However, we will demonstrate that we can correctly evaluate 
probabilistic reachability problems also for certain types of unbounded random variables.

\begin{proposition} \label{prop:inf}
The probabilistic reachability problem for hybrid systems with a single random parameter 
can be correctly solved by a $\delta$-complete decision procedure if:
\begin{itemize}
	\item the domain of the random parameter is bounded from one side,
	\item the domain of the random parameter is unbounded and its probability density 
		function is symmetric.
\end{itemize}
\end{proposition}
\begin{proof}
Let's consider the first case when the domain $\Omega$ of the continuous random variable is bounded from one side. The problem when set $B \subseteq \Omega$ is bounded is trivial and probabilistic reachability problem can be solved correctly by the $\delta$-complete procedure.

If $B$ is unbounded then its complement $\Omega/B$ is bounded (because $\Omega$ is bounded from one side and $B \subseteq \Omega$). Set $\Omega/B$ can be constructed by inverting the relation $\text{unsafe}_{q}(\textbf{r},\textbf{x})$. Taking into account that
\begin{equation} \label{eq:total-probability}
\int_{B} \,dP(r) + \int_{\Omega/B} \,dP(r) = \int_{\Omega} \,dP(r) = 1
\end{equation}
probabilistic reachability problem (\ref{eq:probabilistic-reachability}) is equivalent to
\begin{equation} \label{eq:probabilistic-reachability-one-side}
\exists B_1 \subseteq  \Omega/B: 1 - \int_{B_1} \,dP(r) < C
\end{equation}

Therefore, solving two problems (\ref{eq:probabilistic-reachability}) and (\ref{eq:probabilistic-reachability-one-side}) at the same time by the $\delta$-complete decision procedure guaranties that one of them will terminate with the correct result. Knowing one, we can derive another from the equation (\ref{eq:total-probability}).

Let's consider the second case when $\Omega$ is unbounded and the probability density function is symmetric. We can find two disjoint bounded from one side sets $\Omega^{-}, \Omega^{+} \subset \Omega$ such that $\Omega^{-} \cup \Omega^{+} = \Omega$ and $\int_{\Omega^{-}} \,dP(r) = \int_{\Omega^{+}} \,dP(r) = \frac{\int_{\Omega} \,dP(r)}{2} = 0.5$.

Let $B \subseteq \Omega$. We can find two disjoint sets $B^{-}, B^{+} \subset B$ such that $B^{-} \cup B^{+} = B$, $B^{-} \subseteq \Omega^{-}$ and $B^{+} \subseteq \Omega^{+}$. Then problem (\ref{eq:probabilistic-reachability}) is equivalent to:
\begin{equation} \label{eq:probabilistic-reachability-symmetric}
\exists B_{1}^{-} \subseteq  B^{-}, \exists B_{1}^{+} \subseteq  B^{+} : \int_{B_{1}^{-}} \,dP(r) + \int_{B_{1}^{+}} \,dP(r) \ge C
\end{equation}
where for each of the subsets $B^{-}$ and $B^{+}$:
\begin{equation}
\begin{split}
\int_{B^{+}} \,dP(r) + \int_{\Omega^{+}/B^{+}} \,dP(r)  = 0.5 \\
\int_{B^{-}} \,dP(r) + \int_{\Omega^{-}/B^{-}} \,dP(r)  = 0.5
\end{split}
\end{equation}
If either of subsets $B^{-}$ and $B^{+}$ is unbounded then the technique described above should 
be applied.
\end{proof}

In general, the set $B$ obtained in (\ref{def:Borel-set}) will be of the form:
\begin{equation*} %\label{set-B-one-parameter}
B = \bigcup_{i=1}^{w} B_{i}
\end{equation*}
for some $w \in \mathbb{N}$,
where $B_{i} = [\underline{r}_{i}, \overline{r}_{i}]$ and 
$\forall i \ne j \in \{1,\ldots, w\}:B_{i} \cap B_{j} = \emptyset$. However, if the functions 
representing the dynamics of the system are invertible with respect to the random parameter, 
then set $B$ is formed by a single interval. This allows us to write the computation of integral 
(\ref{eq:probabilistic-reachability}) as a bounded $\Sigma_1$ sentence 
\begin{equation*} %\label{eq:probability-one-variable}
\exists r \in [a, b]: \int_{a}^{r} f_R(x)\, dx \ge C
\end{equation*}
where $f_R$ is the probability density function of the random parameter and $C \in [0,1]$ is a
constant.

The probabilistic bounded reachability problem in hybrid systems with one random initial parameter 
and with invertible dynamics with respect to the random variable can be solved using a validated 
ODE solver that allows encoding integrals as IVPs (initial value problem). We aim for this 
formalisation as that is the way in which dReal handle ODE dynamics.





==> probdeltareach.tex <==
%We now introduce $\delta$-reachability in a probabilistic context.

\begin{definition}\label{def:pHS}
A hybrid system with {\em continuous random initial parameters} consists of $Q$, $X$ and $U$ as in
Definition \ref{def:HS}, and the following components:
\begin{itemize}
%\item $Q = \{q_0, ..., q_m\}$ a set of modes (discrete components of the system),
%\item $X = [u_1, v_1] \times ... \times [u_n, v_n] \times [0, T] \subset \mathbb{R}^{n+1}$ a domain 
	%of continuous variables,
\item $R = [a_1, b_1] \times ... \times [a_l, b_l] \subset \mathbb{R}^{l}$ a domain of {\em random}
	parameters,
\item $S = Q \times R \times X$ is the state space of the system,
%\item $U \subseteq S$ an {\em unsafe} region of the state space,
\end{itemize}
predicates $\text{flow}_{q}(\textbf{r}, \textbf{x}^{0}, \textbf{x}^{t})$,
$\text{init}_q(\textbf{r}, \textbf{x}^{0})$, 
$\text{jump}_{q \rightarrow q'}(\textbf{r}, \textbf{x}^{t}, \textbf{x}^{0})$ and
$\text{unsafe}_{q}(\textbf{r}, \textbf{x}^{t})$.
For all $q\in Q$ the sets defined by $\text{flow}_q, \text{init}_q, \text{jump}_q$,
and $\text{unsafe}_q$ are Borel.
\end{definition}
The random parameters $\mathbf{r}$ are assigned in the initial mode and remain 
unchanged throughout the system's evolution. Also, the
Borel assumption for the sets defined by the predicates is a theoretical requirement for well-definedness
of probabilities, and in practice it is easily satisfied. (We recall that Borel sets are obtained
through countable union and complement of open sets.)

We now modify the bounded $k$ step $\delta$-reachability problem as follows.
\begin{definition}\label{def:probreach}
The bounded $k$ step $\delta$-reachability property for hybrid systems with random initial parameters 
is the bounded $\Sigma_1$ sentence:
\begin{equation*} 
\exists \textbf{r}\   \psi (\textbf{r})
\end{equation*}
where
\begin{equation*} 
\begin{split}
\psi (\textbf{r}) = \exists \textbf{x}^{0}_{0,q_0}, \exists \textbf{x}^t_{0,q_0}, ... , \exists \textbf{x}^{0}_{0,q_m}, \exists \textbf{x}^t_{0,q_m} , ... , \exists \textbf{x}^{0}_{k,q_m}, \exists \textbf{x}^t_{k,q_m}:\\
(\bigvee_{q \in Q} (\text{init}_{q}(\textbf{r}, \textbf{x}^{0}_{0,q}) \wedge \text{flow}_{q}(\textbf{r}, \textbf{x}^{0}_{0,q},\textbf{x}^t_{0,q}))) \\
\wedge (\bigwedge_{i=0}^{k-1} (\bigvee_{q,q' \in Q}(\text{jump}_{q \rightarrow q'}(\textbf{r}, \textbf{x}^t_{i,q}, \textbf{x}^{0}_{i+1,q'}) \\
\wedge (\text{flow}_{q'}(\textbf{r}, \textbf{x}^{0}_{i+1,q'}, \textbf{x}^t_{i+1,q'}))) \wedge (\bigvee_{q \in Q} \text{unsafe}_{q}(\textbf{r}, \textbf{x}^t_{k,q}))))
\end{split}
\end{equation*}

\end{definition}

If we associate a probability measure to the random parameters, then we can assess {\em quantitative} 
system properties (such as the probability that the system reaches the unsafe region).
In particular, we consider the following problem: 
\textit{what is the probability that a hybrid system with random initial parameters reaches the 
unsafe region in $k$ steps?}
To calculate such probability, we first need to find the set 
that contains all the values of the random variables satisfying the reachability property. 
Such a set is constructed as follows:
\begin{equation} \label{def:Borel-set}
B = \{\textbf{r} : \psi(\textbf{r})\}
\end{equation}
where formula $\psi(\textbf{r})$ is per Definition \ref{def:probreach}.
\begin{proposition}\label{prop:BBorel}
The set $B$ defined by (\ref{def:Borel-set}) is Borel.
\end{proposition}
(Proofs can be found in the Appendix.)

The proposition entails that the probability that the system reaches the unsafe region is well-defined. 
Such a probability is computed by integrating the probability measure of  the random variables over 
set $B$. In particular, we need to compute the following integral
\begin{equation} \label{eq:probabilistic-reachability}
\int_{B} \,dP(\textbf{r})\quad  (= \int_{\Omega} I_{U}(\textbf{r})dP(\textbf{r}))
\end{equation}
where $B$ is the set (\ref{def:Borel-set}), $P(\textbf{r})$ is a probability measure over 
the random parameters $\textbf{r}$, $\Omega$ is the support of the random parameters, and 
$I_{U}$ is the indicator function
\begin{equation*}
        I_{U}(\textbf{r}) = 
        \begin{cases}
                1 \quad \text{if the system with parameter $\textbf{r}$ reaches $U$ in $k$-steps} \\
                0  \quad\text{otherwise.}
        \end{cases}
\end{equation*}
If the random parameters are independent then 
$P(\textbf{r}) = \Pi_{i=1}^{l} P_i(r_{i})$, where $P_i$ is the probability measure of 
parameter $r_i$. The infinitesimal probability measure $dP(\textbf{r})$ is usually 
given as a (probability) density function.


